Learning to Repair: Repairing model output errors after deployment using a dynamic memory of feedback

Large language models (LMs), while powerful, are not immune to mistakes, but can be difficult to retrain. Our goal is for an LM to continue to improve after deployment, without retraining, using feedback from the user. Our approach pairs an LM with (i) a growing memory of cases where the user identified an output error and provided general feedback on how to correct it (ii) a corrector model, trained to translate this general feedback into specific edits to repair the model output. Given a new, unseen input, our model can then use feedback from similar, past cases to repair output errors that may occur. We instantiate our approach using an existing, fixed model for script generation, that takes a goal (e.g., "bake a cake") and generates a partially ordered sequence of actions to achieve that goal, sometimes containing errors. Our memory-enhanced system, FBNet, learns to apply user feedback to repair such errors (up to 30 points improvement), while making a start at avoiding similar past mistakes on new, unseen examples (up to 7 points improvement in a controlled setting). This is a first step towards strengthening deployed models, potentially broadening their utility. Our code and data is available at https://github.com/allenai/interscript/.

==> acl-ijcnlp2021-templates/sections-old-v1/UNUSED-from-v2-results.tex <==
% \begin{table}[h]
% \small
% \begin{tabular}{p{0.08\textwidth}p{0.15\textwidth}p{0.07\textwidth}p{0.1\textwidth}}
% \toprule
%  &  Metric & No feedback & w/ general principle \\
% \midrule
% \multirow{2}{*}{Absolute} & Errors per script   & 1.0   & 0.41 \\\cline{2-4}
%                           & Scripts with error  & 100\%    & 75\% \\
% \midrule
% \end{tabular}
% \caption{Is the corrected graph better? \red{Need better caption}. \niket{dataset has only erroneous scripts, fix the first line 1.0. For EMNLP add pos and neg}. TODO2: \niket{comparison with [classification] baseline e.g., classify error type. TODO: why wrong partial order is 100.. also put in counts. Alternative to baseline is to find ablation. for emnlp, with memory can compare with other retrieve / random/ bm25/ }
% }
% \label{tab:results-errors-before-after}
% \end{table}


\section{Preliminary Results}
\label{sec:results}

% \subsection{Initial Results}

\red{Do we evaluate on the test portion of our dataset?}
We evaluate our trained error corrector model $\mathcal{G}$ on the test portion of our dataset.
$\mathcal{G}$ is presented with a script $\tilde{y}$ containing an error, and some general feedback $f$ about the problem.
We wish to evaluate the extent to which
$\mathcal{G}$ can operationalize that feedback and repair the script. Note that both $\tilde{y}$ and the feedback $f$ were unseen during training.

To evaluate the results, we use two metrics: the percentage of local errors that were fixed by the user feedback,
and the number of new errors introduced elsewhere in the graph.
The results are shown in Table \ref{tab:results-errors-before-after},
and indicate that the 59\% of the errors in the scripts were correctly repaired.
\red{PEC: Need to clarify, I don't understand the results table, and how to tell how many new errors were introduced.}
Although preliminary, these results suggest a model can be trained to repair scripts reliably
using natural language feedback.

We also show a categorywise error correction in Table \ref{tab:rq1-ablation-planning}. This indicates that
our corrector model is most effective at understanding and applying feedback about {\bf partial ordering errors},
and struggles the most with feedback about {\bf wrong step ordering}.
\red{Is there an intuitive understanding about why this is?}
\red{PEC: Where did the structure-specific results come from (Table~\ref{results-errors-before-after})?}

% Figure \ref{fig:proscript-instruction-prediction} shows a canonical example of a fixed graph.

\eat{
\begin{figure}[!ht]
\centering
{\includegraphics[width=1.02\columnwidth]{acl-ijcnlp2021-templates/imgs/nl-instruction-prediction-example.png}}
\caption{Model prediction on fixing the script on the left, using the instruction: ``You can't press any buttons if you phone is against your ear''.. The goal here is to make phone call.
% nl instruction=Plan 2 tells you to push the call button after you put the phone to your ear. \\
% General principle instruction=You can't press any buttons if you phone is against your ear.
}
\label{fig:proscript-instruction-prediction}
\end{figure}
}




% Processing predictions/nl_only_pos/dev.nl.tsv
% Before (any-error, %)	24	1.0
% After (any-error, %)	20	0.8333333333333334
% Before (avg-error-per-goal, %)	130	1.0
% After (avg-error-per-goal, %)	68	0.5230769230769231
% predictions/nl_only_pos/dev.nl.tsv	critical_wrong_step(37)	0.3
% predictions/nl_only_pos/dev.nl.tsv	critical_missing_step(28)	0.64
% predictions/nl_only_pos/dev.nl.tsv	critical_wrong_ordering(54)	0.41
% predictions/nl_only_pos/dev.nl.tsv	critical_wrong_flexible_ordering(11)	1.0
% Overall accuracy	0.48

% Processing predictions/nl_only_pos/test.nl.tsv
% Before (any-error, %)	76	1.0
% After (any-error, %)	67	0.881578947368421
% Before (avg-error-per-goal, %)	391	1.0
% After (avg-error-per-goal, %)	202	0.5166240409207161
% predictions/nl_only_pos/test.nl.tsv	critical_wrong_ordering(135)	0.39
% predictions/nl_only_pos/test.nl.tsv	critical_wrong_step(131)	0.27
% predictions/nl_only_pos/test.nl.tsv	critical_wrong_flexible_ordering(44)	0.98
% predictions/nl_only_pos/test.nl.tsv	critical_missing_step(81)	0.72
% Overall accuracy	0.48

% Processing predictions/gp_only_pos/dev.gp.tsv
% Before (any-error, %)	24	1.0
% After (any-error, %)	21	0.875
% Before (avg-error-per-goal, %)	130	1.0
% After (avg-error-per-goal, %)	75	0.5769230769230769
% predictions/gp_only_pos/dev.gp.tsv	critical_wrong_step(37)	0.14
% predictions/gp_only_pos/dev.gp.tsv	critical_missing_step(28)	0.64
% predictions/gp_only_pos/dev.gp.tsv	critical_wrong_ordering(54)	0.39
% predictions/gp_only_pos/dev.gp.tsv	critical_wrong_flexible_ordering(11)	1.0
% Overall accuracy	0.42

% Processing predictions/gp_only_pos/test.gp.tsv
% Before (any-error, %)	76	1.0
% After (any-error, %)	66	0.868421052631579
% Before (avg-error-per-goal, %)	391	1.0
% After (avg-error-per-goal, %)	192	0.49104859335038364
% predictions/gp_only_pos/test.gp.tsv	critical_wrong_ordering(135)	0.47
% predictions/gp_only_pos/test.gp.tsv	critical_wrong_step(131)	0.29
% predictions/gp_only_pos/test.gp.tsv	critical_wrong_flexible_ordering(44)	0.95
% predictions/gp_only_pos/test.gp.tsv	critical_missing_step(81)	0.69
% Overall accuracy	0.51



==> acl-ijcnlp2021-templates/sections-old-v1/abstract.tex <==
\begin{abstract}

Many models produce a structured output, e.g., a graph, an explanation, or a proof, but what does one do when that output contain errors-- can we constantly improve a system through human feedback, without re-training? Our goal is that users could teach a system what the problem is, and what a corrected output with that problem fixed might look like. The model should progressively require less instructions as it learns to generalize from and re-use past instructions.
% Our goal is for users to teach the system what the problem is, and how to correct it, in a way that also generalizes to new problems. 
Our approach is to add an {\it error correction} model, operating on the original model's output. This model is trained on examples of an erroneous output, a general description of the error (stating the general principle that the output violates), and the corrected output. From such examples, the model learns to interpret new natural language error descriptions, and operationalize the corrections that they imply for new outputs. This allows users to correct future new problems in natural language. In addition, by adding a memory of potential problems, the model can recall old problems (corrections) that occur in new examples, and correct those also. The system is trained over a new crowdsourced dataset with 1000 training examples that include natural feedback. This system paves the path towards continuous improvement with progressively less feedback, without retraining.

\end{abstract}

==> acl-ijcnlp2021-templates/sections-old-v1/conclusion.tex <==
\section{Discussion and Conclusion} 
We outline a new system that can perform continuous improvement of the structured output of a model. This is done without retraining, through a memory layer where human feedback is stored and later retrieved efficiently. Our approach generates graphs that have 40\% fewer errors. This work paves a new path towards exciting future research direction of constantly improving the output of NLP models by applying human feedback.


==> acl-ijcnlp2021-templates/sections-old-v1/custom_commands.tex <==
\definecolor{Red}{rgb}{1,0,0}
\definecolor{Green}{rgb}{0.4,1,0.2}
\definecolor{Blue}{rgb}{0,0,1}
\definecolor{Red}{rgb}{0.9,0,0}
\definecolor{Orange}{rgb}{1,0.5,0}
\definecolor{yellow}{rgb}{0.65,0.6,0}
\definecolor{cadmiumgreen}{rgb}{0.2, 0.7, 0.24}
\newcommand{\V}[1]{\mathbf{#1}}
\newcommand{\C}[1]{\mathcal{#1}}
\newcommand{\red}[1]{\textcolor{Red}{#1}}
\newcommand{\green}[1]{\textcolor{cadmiumgreen}{#1}}
\newcommand{\niket}[1]{\textcolor{Red}{[#1 \textsc{--Niket}]}}
\newcommand{\corr}[2]{\textbf{\textcolor{red}{\sout{#1} #2}}}
\newcommand{\pete}[1]{\textcolor{Orange}{[#1 \textsc{--Pete}]}}
\newcommand{\notes}[1]{\textcolor{Red}{[#1 \textsc{--notes}]}}
\newcommand{\ed}[1]{\textcolor{cyan}{[#1 \textsc{--Ed}]}}
\newcommand{\secref}[1]{\S\ref{#1}}
\newcommand\given[1][]{\:#1\vert\:}

% \newcommand{\C}[1]{$\mathcal{#1}$\xspace}

\newcommand{\X}[1]{\mathbf{\mathrm{S}}}
\newcommand{\Z}[1]{\mathbf{\mathrm{C^-}}}
\newcommand{\VV}[1]{\mathbf{\mathrm{C^+}}}
\newcommand{\W}[1]{\mathbf{\mathrm{M^-}}}
\newcommand{\U}[1]{\mathbf{\mathrm{S^-}}}
\newcommand{\Y}[1]{\mathbf{\mathrm{M^+}}}
\newcommand{\LL}[1]{\mathbf{\mathrm{H^-}}}
\newcommand{\M}[1]{\mathbf{\mathrm{H^+}}}
\newcommand{\proscript}[1]{ProScript}


% "Z": [  "C-
%         "V": [ "C+
%         "X": [ "S :
%         "W": [ "M-
%         "U": [ "S- :
%         "Y": [ "M+ :
%         "A": [ "O+ :
%         "D": [ "O+ :
%Constants
\newcommand{\numgraphs}{2107\xspace}
\newcommand{\numpassages}{379\xspace}
\newcommand{\numquestions}{40.7K\xspace}
\newcommand{\grn}[1]{\textcolor{cadmiumgreen}{#1}}


%Hyperparams
\newcommand{\lrate}{\textcolor{Red}{LR-HERE} }
\newcommand{\dropout}{\textcolor{Red}{DROPOUT-HERE} }
% \newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\rdim}[1]{\in \mathbb{R}^{#1}}
\newcommand{\cadmiumgreen}[1]{\textcolor{cadmiumgreen}{#1}}

%\newcommand{\helps}{\stackrel{(+)}\longrightarrow}
% \newcommand{\hurts}{\stackrel{(-)}\longrightarrow}
% \newcommand{\helpedby}{\stackrel{(+)}\longleftarrow}
% \newcommand{\hurtby}{\stackrel{(-)}\longleftarrow}
\newcommand{\helps}{\overset{+}{\longrightarrow}}
\newcommand{\hurts}{\overset{-}{\longrightarrow}}
\newcommand{\helpedby}{\overset{+}{\longleftarrow}}
\newcommand{\hurtby}{\overset{-}{\longleftarrow}}
\newcommand{\entails}{\overset{\oplus}{\longrightarrow}}
\newcommand{\doesnotentail}{\overset{\oplus}{\longleftarrow}}
\newcommand{\relatedby}{\overset{r}{\longrightarrow}}
\newcommand{\ir}{\textsc{ir}\xspace}
\newcommand{\wiqa}{\textsc{wiqa}\xspace}
\newcommand{\quartz}{\textsc{quartz}\xspace}
\newcommand{\quarel}{\textsc{quarel}\xspace}
\newcommand{\defeasible}{\textsc{defeasible}\xspace}
\newcommand{\bert}{\textsc{wiqa-bert}\xspace}
\newcommand{\dotf}{\textsc{dot}\xspace}
\newcommand{\qa}{\textsc{qa}\xspace}
\newcommand{\ours}{\textsc{mercurie}\xspace}  % m explanation reasoning curie
\newcommand{\comet}{\textsc{comet}\xspace}
\newcommand{\plm}{\textsc{plm}\xspace}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\newcommand{\lm}{$\mathcal{L}$\xspace}
\newcommand{\calM}{$\mathcal{M}$\xspace}


\newcommand{\calG}{$\mathcal{G}$\xspace}
\newcommand{\GENS}{$\mathcal{M}^{*}$\xspace}
\newcommand{\GEN}{\calM}
\newcommand{\CORR}{\calG}
\newcommand{\gpt}{\texttt{GPT}\xspace}
\newcommand{\gptt}{\texttt{GPT-2}\xspace}
\newcommand{\tf}{\texttt{T5}\xspace}
\newcommand{\cf}{\textit{cf}\xspace}

\newcommand{\bleu}{\texttt{BLEU}\xspace}
\newcommand{\rouge}{\texttt{ROUGE}\xspace}
\newcommand{\upd}{$\mathbf{S}$\xspace}
\newcommand{\hypo}{$\mathbf{H}$\xspace}
\newcommand{\pre}{$\mathbf{P}$\xspace}
\newcommand{\phu}{$\mathbf{PHS}$\xspace}
\newcommand{\Up}{\textbf{U}\xspace}
\newcommand{\ig}{\textbf{I}\xspace}
\newcommand{\tgen}{\textbf{IGEN}\xspace}
\newcommand{\tgenqa}{\textbf{IGEN-QA}\xspace}
\newcommand{\utype}{\textbf{T}\xspace}
\newcommand{\dquery}{(\pre, \hypo, \upd, \utype)\xspace}

\newcommand{\atomic}{\textsc{atomic}\xspace}
\newcommand{\snli}{\textsc{snli}\xspace}
\newcommand{\social}{\textsc{social}\xspace}
\newcommand{\gengraph}{$\mathbf{G}$\xspace}
\newcommand{\geninfo}{$<$Generated info$>$\xspace}
\newcommand{\sts}{sequence-to-sequence\xspace}
\newcommand{\rqone}{\textsc{rq1}\xspace}
\newcommand{\rqtwo}{\textsc{rq2}\xspace}

\def\@withdot.{\ifmmode\!\string/\!
               \else\kern-1.8pt\string/\kern-1.8pt\fi.}
\newcommand{\inten}{\textit{Intensifies}\xspace}
\newcommand{\atten}{\textit{Attenuates}\xspace}
\newcommand{\dques}{(\pre, \hypo, \upd)\xspace}
\newcommand{\dquesgra}{(\pre, \hypo, \upd, \gengraph)\xspace}
\newcommand{\nle}{\textsc{nl-edit}\xspace}



\newcommand{\squishlist}{
  \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}      \setlength{\parsep}{3pt}
      \setlength{\topsep}{3pt}       \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{1.5em} \setlength{\labelwidth}{1em}
      \setlength{\labelsep}{0.5em} } }
\newcommand{\reallysquishlist}{
  \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}    \setlength{\parsep}{0pt}
      \setlength{\topsep}{0pt}     \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{0.2em} \setlength{\labelwidth}{0.2em}
      \setlength{\labelsep}{0.2em} } }

 \newcommand{\squishend}{
     \end{list} 
 }

 

==> acl-ijcnlp2021-templates/sections-old-v1/feedback.tex <==
\section{Human feedback on $\mathcal{M}$}
\label{sec:feedback-proscript}

% \begin{figure*}[!ht]
% \centering
% {\includegraphics[width=0.7\textwidth]{acl-ijcnlp2021-templates/imgs/feedback-examples.png}}
% \caption{Examples of feedback on scripts. First line shows the natural language feedback and below it is a generalized version that annotators were asked is like explaining to a five year old. \red{reformat as a table}}
% \label{fig:proscript-feedback-examples}
% \end{figure*}



\begin{figure*}[!ht]
\centering
{\includegraphics[width=0.7\textwidth]{acl-ijcnlp2021-templates/imgs/feedback-examples.png}}
\caption{Examples of feedback on scripts. First line shows the natural language feedback and below it is a generalized version that annotators were asked is like explaining to a five year old. TODO: reformat as a table}
\label{fig:proscript-feedback-examples}
\end{figure*}

The annotators were instructed to describe the errors in the script as generally as possible. We first asked the annotator to describe the error in natural language, and then asked them how they would explain it to a five year old (this simplified and generalized feedback is the final outcome of this annotation task). The Turkers were asked to ignore grammatical and fluency errors, and focus on critical errors of four types:
\squishlist
\item Wrong ordering: the order in the sequence of steps is not correct (e.g., wearing shoes is described before wearing socks).
\item Flexible ordering: some steps can be done in a flexible order (e.g., you can wear left sock or right sock first). A bad plan usually does not depict such flexibility.
\item Missing critical steps: a bad plan might have missed critical steps (e.g., the plan can say: "wait for a plane" followed by "get off the plane" -- here an obvious step "get on the plane" is missing) . There is no strict definition for a critical step, so use your gut feeling.
\item Wrong step: a bad plan might have irrelevant and wrong steps (e.g., the plan describing "go to a party" might describe an irrelevant step such as read a book, open a book etc.).
\squishend



% \begin{figure}[!ht]
% \centering
% {\includegraphics[scale=0.5]{acl-ijcnlp2021-templates/imgs/proscript-sample.png}}
% \caption{A data point from an automatically generated script. Steps 4,5 and 4,6 have a wrong ordering, hence the feedback is: \textit{People must get into a vehicle, before driving to any place}. Details of how we acquire such feedback is in Sec. \ref{sec:feedback-proscript}}
% \label{fig:example-graph-fixed}
% \end{figure}







% Less Non-critical errors: These characteristics do not define a worse plan::
% Grammatical and fluency errors: a bad plan usually has less fluent steps or contains many grammatical mistakes.
% Redundant steps: some steps in the plan might have redundant steps, e.g., step 3 and step 4 might repeat.
% Granularity: note that a more fine-grained plan is not a worse plan (e.g., go the bed, get up, go brush vs. get up, get ready)


Annotators were required to list only one critical error that they believe was most important. Each data point is annotated by three annotators, adding some diversity in the errors (more than one errors were annotated in about 60\% of the examples. % TODO Niket confirm this stat.
Figure \ref{fig:proscript-feedback-examples} presents some random examples of feedback, collating wrong ordering and wrong flexible ordering as edge error, and missing step and step error as node error.



==> acl-ijcnlp2021-templates/sections-old-v1/introduction.tex <==
\section{Introduction}
Teaching a machine via human instructions has long been a goal of AI, yet current neural methods typically require large numbers of examples to convey knowledge. Recently, LeapOfThought \cite{Talmor2020TeachingPM} instead taught pre-trained models on-the-fly using a few general statements without requiring re-training of the model. For the first time we \textit{attempt} to continuously teach a neural model through corrections on its output structure with a memory based architecture that avoids re-training. 


\begin{figure}[!ht]
\centering
{\includegraphics[width=\columnwidth]{acl-ijcnlp2021-templates/imgs/example-graph.png}}
\caption{Left: An automatically generated noisy script. Steps 4,5 and 4,6 have a wrong ordering, hence the general principle based feedback is: \textit{People must get into a vehicle, before driving to any place}. Right: the corrected graph. Acquisition of such feedback data is in \S \ref{sec:feedback-proscript}. Fixing the graph is in \S \ref{sec:method} }
\label{fig:intro-example}
\end{figure}

% Niket: An extended related work discussion here to dispense with the related work.
A common theme in prior approaches to this task based on interactive semantic parsing (such as \cite{elgohary2021nl, percy-2016-learning-language-games-interaction-shouldrn}) is that user feedback is mapped into structure edit commands, which can then be executed on the incorrect structures to fix it. For example, \cite{elgohary2021nl} presented \nle to fix SQL queries using human feedback such as: 
\texttt{replace course id with program id.}. 
However:
\squishlist
\item the feedback are syntactic with a certain task-specific formal structure, e.g., \nle is known to struggle with natural feedback that does not describe an edit directly \cite{elgohary2021nl}.
\item the feedback is expected to be actionable. Rather than highlighting a problem or error, it is expected to contain a solution to fix the error. This feedback is then parsed using semantic parsing techniques into a set of structure edit commands. 
\item past feedback is discarded, and not used in future examples. In practice, a system often encounters recurring themes or situations, or nearly similar situations, e.g., \textit{people must get into a vehicle before driving to any place}. 
\squishend

Overcoming these problems, this paper does not make assumptions about the structure of the feedback and gives flexibility to a human to supply natural language instructions which could point out to some error and not necessarily edit specifications. This allows the editing operations to be inferred implicitly, triggered by the specification of the error. 

We propose a pipeline system with two components, a previously trained neural model $\mathcal{M}$ and a graph corrector $\mathcal{G}$. The system takes as input any previously trained neural model $\mathcal{M}$ capable of generating a structured output. The second input is a natural language human feedback on the output structure (for an example, see Figure \ref{fig:intro-example}). As output, it produces a better structure, without retraining using a feedback table accessible through a memory layer.



==> acl-ijcnlp2021-templates/sections-old-v1/method.tex <==
\section{Method}
\label{sec:method}

We propose a pipeline system with two components, a previously trained neural model $\mathcal{M}$ and a graph corrector $\mathcal{G}$. The second input is a natural language human feedback on the output structure. As output, it produces a better structure, without retraining using a feedback table accessible through a memory layer.

\begin{figure}[!ht]
\centering
{\includegraphics[width=\columnwidth]{acl-ijcnlp2021-templates/imgs/pipeline.pdf}}
\caption{Our pipeline: the output generated by \GEN is corrected by \CORR using human feedback. TODO: show memory}
\label{fig:pipeline}
\end{figure}


See Algorithm \ref{alg:alg-1} for an outline of the method.

\SetKwRepeat{Do}{do}{while}
\SetKwInput{KwGiven}{Given}
\SetKwInput{KwInit}{Init}
\SetKwInput{KwTrainCorr}{Training}
\SetKwInput{KwInference}{Inference}
\begin{algorithm}[!ht]
\SetAlgoLined
\KwGiven{\GEN: $x_i \rightarrow  \tilde{y_i}$ ; feedback table $\mathcal{T} = \emptyset$} 
\vspace{0.7em}
\KwTrainCorr{}
\Indp
$\mathcal{D}_{\mathcal{G}} = \emptyset$\;
\For{$i \gets 1, 2, \ldots, N$}{
$\tilde{y}_i = \mathcal{M}(x_i)$ [build cache]\;
$I_i = \texttt{feedbk}(\tilde{y}_i)$ [from train data]\;
$\mathcal{T} = \mathcal{T} \cup (x_i, \tilde{y}_i, I_i)$ [build table]\;
}
\For{$j \gets 1, 2, \ldots, N$}{
\textbf{$\mathcal{I'}$} = $\texttt{attend} (\tilde{y}_i, \mathcal{T})$ [retrieve]\;
$\hat{y_i} = \mathcal{G} (\tilde{y}_i$, $\mathcal{I'}$) [corrector output]\;
${y_i}^* = \texttt{gate} (\tilde{y}_i$, $\hat{y}_i$) \;
$\mathcal{L} += \texttt{dist}({y_i}^*, y_i) + rank(I_j, \mathcal{I'})$ 
}

\Indm
\vspace{0.7em}
% \KwInference{}
% \Indp

% $\tilde{y} = \mathcal{M}(x)$\;
% \While{$I: \texttt{attend}(\tilde{y}) \neq \emptyset$} {
% $\tilde{y} = \mathcal{G}(x, I, \tilde{y})$\;
% }
% $y = \tilde{y}$\;
\caption{Our algorithm with memory store to correct output through feedback}
\label{alg:alg-1}
\end{algorithm}





==> acl-ijcnlp2021-templates/sections-old-v1/old-experiments.tex <==
\section{old Experiments}

\begin{table*}[!h]
    \centering
    \begin{tabular}{l|l|l}
    \toprule
    \small{model} & \small{input  →  output} & \small{ROUGE} \\
    \midrule
    \small{no-fb} & $x \rightarrow y$ &  31.16 \\ % / 31.28 \\ 
    \small{rndm-fb} & $x + fb_{rndm} \rightarrow y$ &  32.1 \\ % This is approximate from the top of the head % / 31.28 \\ 
    % \ours $+ fb_i$         & $x + fb_i + \Omega_{attn}{(fb_{1..T})} \rightarrow y$              &  56.16 \\ %/50.15
    \small{with-fb}       & $x + fb_i \rightarrow y$                              &  57.10 \\  %/48.82 
    \midrule
    \small{train-fb knn}  & $x + \Omega_{knn}{(fb_{1..T})} \rightarrow y$ &  27.73 \\ % / 30.87 \\
    \small{train-fb attn} & $x + \Omega_{attn}{(fb_{1..T})} \rightarrow y$ &  33.60 \\ % / 30.87 \\
    \midrule
    \small{train-test-fb knn}   & $x +  \Omega_{knn}{(fb_{1..T}, fb_{1..{i-1}})} \rightarrow y$ &  31.86 \\ % / 30.87
    \small{train-test-fb attn}  & $x + \Omega_{attn}{(fb_{1..T}, fb_{1..i-1})} \rightarrow y$ &  33.60 \\ %/ 31.25
    \midrule
    && \\
    &Adding bad feedback hurts& \\
    \small{train-fb knn + $fb_i$} & $x + fb_i + \Omega_{knn}{(fb_{1..T})}  \rightarrow y$ &  40 \\ % / 30.87 \\
    \small{train-test-fb knn  + $fb_i$}  & $x + fb_i + \Omega_{knn}{(fb_{1..T}, fb_{1..i})}  \rightarrow y$ &  47 \\ % / 30.87 \\
    % \baselinebart $+ fb_i$       & $x + fb_i \rightarrow y$                              &  57.10 \\  %/48.82 
    \midrule
    && \\
    &Oracle retrieval (different fb representation)& \\
    \small{with-fb oracle attn} & $x + \Omega_{attn}{gold}  \rightarrow y$ &  34 \\ % / 30.87 \\
    \small{with-fb oracle attn} & $x + \Omega^{fb-seq-rep}_{attn}{gold}  \rightarrow y$ &  55 \\ % / 30.87 \\
    \end{tabular}
    \caption{Main results table}
    \label{tab:results_main}
\end{table*}

\paragraph{TODOs}
\squishlist
\item We should add no feedback.
\item The aspect of the x query and x memory that kNN compares on, is not about badness.
\squishend

\begin{table*}[]
\centering
\begin{tabular}{@{}ll@{}}
\toprule
\textbf{Error-identifiability (EI)} & \begin{tabular}[c]{@{}l@{}}There should exist a method that can: i) successfully identify $\V{e}_i$, and ii) access\\ memory based on $\V{e}_i$ to retrieve useful feedback.\end{tabular}                                            \\ \midrule
\textbf{Exchangeability (EX)} & \begin{tabular}[c]{@{}l@{}}If $\V{x}_i$ and $\V{x}_j$ have similar errors (i.e., $\V{e}_i \sim \V{e}_j$), then the feedbacks $\V{fb}_i$ and $\V{fb}_j$\\ should be \textit{exchangeable}  (i.e., $\V{x}_i$ should be correctable with $\V{fb}_j$ and vice-versa.) Another way to put this would be that proximity of errors should imply proximity of feedbacks $(e_i ~ e_j \implies fb_i \sim fb_j)$. \end{tabular} \\ \midrule
\textbf{Non-sufficiency (NS)} & \begin{tabular}[c]{@{}l@{}}If true feedback $\V{fb}_i$ is available during inference, then it should not be sufficient to\\ fix the error: the model/dataset should leverage and benefit from multiple related\\ feedbacks, which the dataset should contain (by exchangeability) and the model\\ should successfully recover (error-identifiability).\end{tabular} \\
\bottomrule
\end{tabular}
\caption{The memory checklist: a set of necessary conditions for the dataset and model for any auxiliary memory setup to be useful. We assume a general setup in which an input $\V{x}_i$ has an error $\V{e}_i$, which can be corrected using feedback $\V{fb}_i$ to generate a correction $\V{y}_i$. The memory consists of a set of feedbacks $\{\V{fb}_i\}$.}
\end{table*}





% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[]
\centering
\begin{tabular}{@{}lll@{}}
\toprule
ExpId & Model                                                                          & ROUGE \\ \midrule
1 & Bad plan + true feedback [string]                                              & 55    \\
2 & Bad plan + true feedback [EOS]                                                 & 30    \\
3 & Bad plan + true feedback [All hidden states]                                   & 52    \\
4 & Bad plan + true feedback [All hidden states] + feedback of k nearest bad plans & 47 (with-cutoff)   \\
5 & Bad plan + feedback of k nearest bad plans & ?   \\
6 & Bad plan + feedback of k nearest bad plans [all hidden states] & ?     \\
\bottomrule
\end{tabular}
\caption{Plan of experiments. True feedback [EOS] is implemented using Oracle attention.}
\label{tab:variations}
\end{table*}


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[]
\centering
\begin{tabular}{@{}ll@{}}
Id & Next steps                   \\ 
\midrule
  1 & Learn attention or k-nearest parameters \\
  2 &  We should add no feedback. \\
  3 &  The aspect of the x query and x memory that kNN compares on, is not about badness.                          \\
  4 &  expect the model to attend to one feedback (reinforcing the same thing is not helping the model) \\
   &                              \\ \bottomrule
\end{tabular}
\caption{}
\label{tab:ideas}
\end{table*}

\begin{table}[!h]
    \centering
    \begin{tabular}{l|l|l}
    \toprule
    \small{model} & \small{input  →  output} & \small{accuracy} \\
    \midrule
    \baselinebart $+ fb_i/10$       & $x + fb_i/10 \rightarrow y$                        &  xxx \\ 
    \baselinebart $+ fb_i/50$       & $x + fb_i/50 \rightarrow y$                        &  xxx \\ 
    \baselinebart $+ fb_i$       & $x + fb_i \rightarrow y$                              &  xxx \\ 
    \midrule
    \ours $+ fb_{1..i/10}$       & $x + \omega{(fb_{1..T}, fb_{1..i/10})} \rightarrow y$ &  xxx \\
    \ours $+ fb_{1..i/50}$       & $x + \omega{(fb_{1..T}, fb_{1..i/50})} \rightarrow y$ &  xxx \\
    \ours $+ fb_{1..i}$          & $x + \omega{(fb_{1..T}, fb_{1..i})} \rightarrow y$    &  xxx \\ 
    \midrule
    \end{tabular}
    \caption{Evolving results table}
    \label{tab:results_evolving}
\end{table}


Now, we discuss the following three questions:

\paragraph{Q1: Does \ours increase accuracy?} 
\niket{show examples, discuss numbers in Table \ref{tab:results_main}} Discuss if just memory helps, and if adding memory model to the baseline with fb helps.

\paragraph{Q2: Is \ours interpretable?} 
\niket{TODO: show examples of attended feedbacks being relevant or not} Are the feedbacks retrieved from the memory reasonable?

\paragraph{Q3: Is \ours using past feedback effectively?}    
\niket{TODO: show examples and numbers as memory grows incl at test} incrementally add the test feedback to memory, and allow the subsequent examples to attend over them. We could find 5 good examples and 2 bad examples. 


\subsection{Error Analysis}
\squishlist

\item \textbf{Type of edit}: Some edit types are more difficult than others. Examples ...

\begin{table}[!h]
\small
\begin{tabular}{ll}
\toprule
Target error type & Accuracy  \\
\midrule
Wrong step error   & xxx    \\
Missing step error   & xxx \\
Wrong order      & xxx  \\
Wrong partial order   & xxx  \\
\midrule
Overall   & xxx  \\
\midrule
\end{tabular}
\caption{type of edit analysis table}
\label{tab:analysis-type-of-edit}
\end{table}

\item \textbf{Component of edit}: Identifying the type of edit vs the argument of the edit. TODO: ... Examples ...

\item \textbf{Attention}: errors as a result of attending to wrong feedback? TODO: ... Examples ...
    
\squishend


























% NOTES in experiment section
% \niket{
% main table of results:
% Feedback with oracle memory → ideal feedback with best top-1 retrieval (upper bound) (assuming one feedback helps, but maybe memory would do better by attending to past)
% Feedback with attended memory → bad graph [+ retrieved feedback] → edit .. Model has learned to interpret retrieved feedback.
% No feedback: bad graph → edit}

% \niket{dataset: WIQA may not be goal-oriented. (can mention as a small contribution).
% question: can G be used on a new domain (would retrieve feedback relevant to proscript --- though goals and actions are general). e.g., relabel an edge.}
% \niket{
% main analysis:
% ablation analysis -- what helps.
% error analysis
% memory analysis (top-3 feedbacks) -- which feedbacks 
% }





% \begin{enumerate}
%     \item \red{included} \textit{FEEDBACK HELPS} Does feedback help in generating correct edits? Or is the model able to figure out the problem with the bad plan and generate the edit? (no feedback at all vs. true feedback). We must clearly answer and highlight this. 

%     \item \red{included} \textit{FEEDBACK + MEMORY HELPS} In addition to the true feedback, does a memory of feedback help in generating better edits? (true feedback vs. true feedback + memory).

%     \item \red{included} \textit{JUST MEMORY HELPS} How useful is memory without the true feedback? (at test time, only use the train + dev memory).
    
%     \item \red{included} \textit{MEMORY HELPS IN LOW DATA SETTINGS} Does memory help in alleviating data sparsity? In order to show this, we will experiment with ${10\%, 20\%, 30\%, \ldots, 100\%}$ of the data with and without memory. 

%     \item \red{included} \textit{GROWING THE MEMORY AT TEST TIME HELPS} Does growing the memory help? To answer this question, we incrementally add the test feedback to memory, and allow the subsequent examples to attend over them. Intuitively, this should be the best performing model.
    
%     \item  \red{skipped}  \textit{DOES RETRAINING IMPROVE OVER GROWING MEMORY?} Once the memory has grown to a certain extent, what would be get by re-training? This can be simulated as follows: i) Run the process to the end by using the dev set (i.e., grow the memory using dev-set). Then retrain the system with train + dev, and evaluate on test. Is this better than continuously growing the memory?
  
%     \item \red{included} \textit{INTERPRETABILITY} Are the feedbacks retrieved from the memory reasonable?
        
% \end{enumerate}




==> acl-ijcnlp2021-templates/sections-old-v1/old-method.tex <==







% \paragraph{Necessary conditions:} The necessary conditions for any such auxiliary memory setup to be useful are as follows. 

% \squishlist
% \item \textbf{Implied-error based retrieval (identifiability)}: The method must: (i) (latently) infer the implied error $\V{e}_i$, and (ii) access memory based on $\V{e}_i$ to retrieve feedback that applies to the implied error.
% Any method that hopes to fix a problem must first uncover the error. Thus, identifiability is the first necessary condition.

% \item \textbf{Feedback exchangeability}: If $\V{x}_i$ and $\V{x}_j$ have similar errors (i.e., $\V{e}_i \sim \V{e}_j$), then their feedbacks $\V{fb}_i$ and $\V{fb}_j$ should be exchangeable (i.e., $\V{fb}_j$ should apply to $\V{x}_i$.), i.e., $(e_i \sim e_j \Leftrightarrow fb_i \sim fb_j)$

% % Put differently, the proximity of errors should imply proximity of feedbacks and vice-versa $(e_i \sim e_j \Leftrightarrow fb_i \sim fb_j)$

% % \item \textbf{Non-sufficiency}: 
% \item \textbf{Redundancy}: Even if $\V{fb}_i$ directly applies to $\V{x}_i$, adding $\V{fb}_j$ such that $fb_i \sim fb_j)$ should benefit the model.


% % If true feedback $\V{fb}_i$ is available during inference, then it should not be sufficient to fix the error: the model/dataset should leverage and benefit from multiple related feedbacks, which the dataset should contain (by exchangeability) and the model should successfully recover (error-identifiability)

% \squishend




==> acl-ijcnlp2021-templates/sections-old-v1/results.tex <==
\section{Results}
\label{sec:results}


We setup experiments to judge whether our method was effective. We count the percentage of local errors that got fixed and new errors introduced elsewhere in the graph, see Table \ref{tab:results-errors-before-after}. We also show a category wise error correction in Table \ref{tab:rq1-ablation-planning}. Figure \ref{fig:proscript-instruction-prediction} shows a canonical example of a fixed graph.

\begin{table}[!h]
\small
\begin{tabular}{p{0.08\textwidth}p{0.15\textwidth}p{0.07\textwidth}p{0.1\textwidth}}
\toprule
 &  Metric & No feedback & w/ general principle \\
\midrule
\multirow{2}{*}{Absolute} & Errors per script   & 1.0   & 0.41 \\\cline{2-4}
                           & Scripts with error  & 100\%    & 75\% \\
\midrule
\end{tabular}
\caption{Is the corrected graph better?}
\label{tab:results-errors-before-after}
\end{table}

\begin{figure}[!ht]
\centering
{\includegraphics[width=1.02\columnwidth]{acl-ijcnlp2021-templates/imgs/nl-instruction-prediction-example.png}}
\caption{Model prediction on fixing the script on the left, using the instruction: ``You can't press any buttons if you phone is against your ear''.. The goal here is to make phone call.
% nl instruction=Plan 2 tells you to push the call button after you put the phone to your ear. \\
% General principle instruction=You can't press any buttons if you phone is against your ear.
}
\label{fig:proscript-instruction-prediction}
\end{figure}


\begin{table}[]
\small
\begin{tabular}{lll}
\toprule
Feedback type &  Target error type & \% Target fixed \\
 &  (task specific) & (higher is better)  \\
\midrule
\multirow{2}{*}{Generic} & Wrong step error   & 42\%    \\
                         & Missing step error   & 81\% \\
                         & Wrong order      & 47\%  \\
                         & Wrong partial order   & 100\%  \\
                         \midrule
                         & Overall   & 59\%  \\
\midrule
\multirow{2}{*}{Structure specific} & Wrong step error   & 50\% \\
                         & Missing step error   & 81\%     \\
                         & Wrong order   & 50\%    \\
                         & Wrong partial order   & 100\% \\
                         \midrule
                         & Overall   & 62\%  \\
\midrule
\end{tabular}
\caption{ablation table for planning task}
\label{tab:rq1-ablation-planning}
\end{table}




% Processing predictions/nl_only_pos/dev.nl.tsv
% Before (any-error, %)	24	1.0
% After (any-error, %)	20	0.8333333333333334
% Before (avg-error-per-goal, %)	130	1.0
% After (avg-error-per-goal, %)	68	0.5230769230769231
% predictions/nl_only_pos/dev.nl.tsv	critical_wrong_step(37)	0.3
% predictions/nl_only_pos/dev.nl.tsv	critical_missing_step(28)	0.64
% predictions/nl_only_pos/dev.nl.tsv	critical_wrong_ordering(54)	0.41
% predictions/nl_only_pos/dev.nl.tsv	critical_wrong_flexible_ordering(11)	1.0
% Overall accuracy	0.48

% Processing predictions/nl_only_pos/test.nl.tsv
% Before (any-error, %)	76	1.0
% After (any-error, %)	67	0.881578947368421
% Before (avg-error-per-goal, %)	391	1.0
% After (avg-error-per-goal, %)	202	0.5166240409207161
% predictions/nl_only_pos/test.nl.tsv	critical_wrong_ordering(135)	0.39
% predictions/nl_only_pos/test.nl.tsv	critical_wrong_step(131)	0.27
% predictions/nl_only_pos/test.nl.tsv	critical_wrong_flexible_ordering(44)	0.98
% predictions/nl_only_pos/test.nl.tsv	critical_missing_step(81)	0.72
% Overall accuracy	0.48

% Processing predictions/gp_only_pos/dev.gp.tsv
% Before (any-error, %)	24	1.0
% After (any-error, %)	21	0.875
% Before (avg-error-per-goal, %)	130	1.0
% After (avg-error-per-goal, %)	75	0.5769230769230769
% predictions/gp_only_pos/dev.gp.tsv	critical_wrong_step(37)	0.14
% predictions/gp_only_pos/dev.gp.tsv	critical_missing_step(28)	0.64
% predictions/gp_only_pos/dev.gp.tsv	critical_wrong_ordering(54)	0.39
% predictions/gp_only_pos/dev.gp.tsv	critical_wrong_flexible_ordering(11)	1.0
% Overall accuracy	0.42

% Processing predictions/gp_only_pos/test.gp.tsv
% Before (any-error, %)	76	1.0
% After (any-error, %)	66	0.868421052631579
% Before (avg-error-per-goal, %)	391	1.0
% After (avg-error-per-goal, %)	192	0.49104859335038364
% predictions/gp_only_pos/test.gp.tsv	critical_wrong_ordering(135)	0.47
% predictions/gp_only_pos/test.gp.tsv	critical_wrong_step(131)	0.29
% predictions/gp_only_pos/test.gp.tsv	critical_wrong_flexible_ordering(44)	0.95
% predictions/gp_only_pos/test.gp.tsv	critical_missing_step(81)	0.69
% Overall accuracy	0.51

==> acl-ijcnlp2021-templates/sections-old-v1/task_dataset.tex <==
\section{Task and starting model $\mathcal{M}$}

\subsection{Structured prediction task}
\label{sec:task-proscript}
In principle, we could consider any structured task. In this paper, we consider script generation. \textit{Scripts}, introduced by \newcite{Schank1975ScriptsPA}, represent structured commonsense knowledge about prototypical events in everyday situations/scenarios such as \textit{bake a cake} and \textit{fuel a car}. There are several variations for script knowledge representation, we consider ProScript \citet{proscript}, which is similar to \newcite{regneri-etal-2010-learning} rather than \textit{narrative chain}~\cite{chambers-jurafsky-2008-unsupervised}. ProScript is a recently introduced dataset, where the task is to generate a partial order script given a goal. The script generation task takes a goal as input and the output is a partial order script $G(V, E)$, where $V$ is a set of essential events $\{v_1, ... v_i, ... v_{|V|}\}$ and $E$ is a set of temporal ordering constraints between events $\{e_{ij}\}$ which means that the events $v_i$ must precede the event $v_j$ ($v_i \prec v_j$). That is, models are required to \textit{generate} events ($V$) and predict the edges ($E$) jointly. 

\subsection{Design of $\mathcal{M}$}
In principle, $\mathcal{M}$ can be any model that is capable of generating a structured output, e.g., an encoder decoder architecture such as BART, T5, etc. In this study, $\mathcal{M}$ is the recently published \cite{proscript} (strongest) baseline on \texttt{proScript}. $\mathcal{M}$ is based on T5 \cite{raffel2020exploring}, which is an encoder-decoder model, that translates any task as a text-to-text generation. $\mathcal{M}$ was trained on \texttt{proScript}~\cite{proscript} dataset, which consists of 6.4k of crowdsourced partially ordered scripts. In that dataset, scenarios are extracted from ROCStories~\cite{mostafazadeh-etal-2016-corpus}, DeScript~\cite{wanzare-etal-2016-crowdsourced}, and Virtual-Home~\cite{puig2018virtualhome}, and crowd workers generate partially ordered scripts for these scenarios. Next, we create a new dataset that contains human feedback on the output of $\mathcal{M}$. 


==> sections/abstract-old-v1.tex <==
\begin{abstract}

% \niket{todo: point out that the base model produces commonsense mistakes in the title and abstract} Large LMs, while powerful, are not immune to mistakes, but are prohibitively costly to retrain. Our goal is to allow users to correct such errors directly through interaction -- without retraining -- by giving feedback on the model's beliefs or explanations. We create a dynamic memory architecture... with a growing memory of cases where the model misunderstood the user's intent and was provided with feedback. Given a new query, our memory-enhanced model uses feedback from similar, prior queries to enrich the input. We show empirically that this works on a structured prediction real task. memory helps avoid repeating similar past mistakes. Our simple idea is a first step towards strengthening deployed models, potentially broadening their utility. 

How can an end-user provide feedback if a deployed structured prediction model generates incorrect output? Our goal is to allow users to correct errors directly through interaction, without retraining, by giving feedback on the model's output. We create a dynamic memory architecture with a growing memory of feedbacks about errors in the output. Given a new, unseen input, our model can use feedback from a similar, past erroneous state. On a script generation task, we show empirically that the model learns to apply feedback effectively (up to 30 points improvement), while avoiding similar past mistakes after deployment (up to 10 points improvement on an unseen set). This is a first step towards strengthening deployed models, potentially broadening their utility. 

% Peter's comments
% Re-use notations from GPT-3?
% frame in terms of interactive feedback (introduction)
% 

% Given a partially incorrect structure and end user feedback, we aim to localize an erroneous node or edge in the graph and generate a repaired graph. Learning structure repair has two major challenges: First,
% the system needs to connect and jointly reason over the incorrect source structure and the user feedback. Second, existing works do not account for end-user feedback after deployment (e.g., expert feedback, rather than end user feedback, is used in natural language database query parsing \citep{elgohary2021nl}; and compiler feedback is used for code fixing in  \citet{Yasunaga2020Bifi-v0-PercyLiang} but this severely limits the generality of their approaches). End users typically may not know the completely correct output structure but can critique on any inconsistencies or commonsense issues in partially correct output structures (common in practice). Our key innovation is modeling of post deployment structured output repair with a dynamic feedback memory architecture.

% \textbf{\red{TODOs}}: 
% \begin{enumerate}
%     \item do we need more tasks (in this paper: speculate requirements of this task e.g, feedback can be expressed in a general way.. not an parse-able feedback.. try the proofwriter .. there is no question+feedback.. we can enrich existing dataset with question context simpler structure and  ... ) .. applying to entailment writer domain? 
%     \item this paper should have a very general architecture. there are two ways of applying feedback so there are two architecture (maybe a caveat that the other setup requires more training examples) it still caters to the general story that we modify behavior without retraining. 
%     \item It would be interesting to compare gold and retrieved feedback (IR PERF). 
%     \item since openpi qa is difficult to collect right now (for every step in the script ... we can do verification over the possibilities... is this step relevant to the goal and does not evaluate the flow (train a new multitasking angle for this). We could atleast use it as a metric to score scripts. Train on samples from openpi (negative samples have steps from irrelevant or from similar looking scripts -- T5. probably goal, step, is relevant label. \am{irrelevant steps dataset})

% \end{enumerate}

% \textbf{Empirical backup of the story:} Improving model accuracy (7\% currently with a potential of up to 27\% with good retrieval) through a memory of feedbacks on a structured prediction task of script generation. The task setup is general; it takes in a structure as input and outputs a structure. Specifically:

% \begin{enumerate}
% \item \textbf{[motivation]} gpt3 memprompt like experiment does not work with interscript: for tasks that require more examples (one use case in this paper), in-prompt learning is not sufficient to give feedback on the fly. %(memprompt/gpt3_interscript.py) and https://docs.google.com/document/d/12pAQKFpxViPQ3abqdyJFv-Jk1fGrCU2ln1woYRA34SM/edit
% % From the FLAN paper. Although they claim that “few-shot is better for large/complex output spaces,” the examples they quote are not quite large or complex. This is also the opposite of what you found with GPT-3 for script generation.
% \item \textbf{[model]} that uses feedback: the model learns to apply (non-actionable) feedback to generate a better script graph.
% \item \textbf{[dynamic memory]} the memory dynamically grows with user interactions. We also discuss some assumptions on feedback so that the memory becomes useful -- e.g., feedback exchangeability across similar examples. 
% \item \textbf{[results]} The T5 based model has learned to apply feedback with an accuracy of more than 70\% . In a multitasking setup, our model is able to generate a script given a goal, and correct it using natural feedback. On the interaction set, the model is able to improve by 7\% on unseen instances at test time just by maintaining the memory from training (baseline trained model that uses no explicit feedback is at 63.9\%). If the BERT based memory lookup is replaced by oracle retrieval, the gains go up to 28\% . 
% \item \textbf{[future directions]} Improving the IR can give us even bigger gains. Further, the multitasking setup is showing that more reasoning can be done e.g., being selective about applying  feedback and more consistency across these different tasks/ angles.
% \end{enumerate}

% Given an erroneous output, our goals are two-fold: first, to enable a user to give a natural language feedback describing the error; and second, the ability to recall relevant old corrections so that new examples can generalize from past corrections. We propose a model that is trained on examples of erroneous output and necessary corrections, and effectively attends over a memory store of feedbacks. This model is interpretable (it gives the feedbacks that contributed to the correction), evolving (the memory store grows over time). We show that the model is effective on an existing script generation task as it can repair script errors through natural feedback (e.g., you must get in a car to drive somewhere); and  uses past feedback to generalize to new examples. This paves a path towards continuous improvement, without requiring retraining. 




% Many models produce a structured output, e.g., a graph, an explanation, or a proof, but what does one do when that output contains errors - can we constantly improve a system through human feedback, without re-training? Our goal is that users could teach a system what the problem is, and what the required correction should be. We also should be able to recall relevant old problems (corrections) so that new examples can generalize from past corrections, paving a path towards continuous improvement with progressively less feedback. Our approach is to add an {\it error correction} model, operating on the original model's output. This model is trained on examples of an erroneous output, a general description of the error (stating the general principle that the output violates), and required corrections. Our model architecture includes a memory of users' feedback, so that the model can recall old problems (corrections). We show results on an existing task of generating {\it scripts} (a graph of event sequences including partial order), and find that the model is able to repair script errors through natural feedback (e.g., on wrong event ordering). We also show that the model can effectively use past memory of feedbacks; and this itself leads to a 5\% ROUGE absolute improvement.
\end{abstract}






% \begin{abstract}

% Many models produce a structured output, e.g., a graph, an explanation, or a proof, but what does one do when that output contain errors - can we constantly improve a system through human feedback, without re-training? Our goal is that users could teach a system what the problem is, and what a corrected output with that problem fixed might look like. The model should progressively require less instructions as it learns to generalize from and re-use past instructions.
% % Our goal is for users to teach the system what the problem is, and how to correct it, in a way that also generalizes to new problems. 
% Our approach is to add an {\it error correction} model, operating on the original model's output. This model is trained on examples of an erroneous output, a general description of the error (stating the general principle that the output violates), and the corrected output. From such examples, the model learns to interpret new natural language error descriptions, and operationalize the corrections that they imply for new outputs.
% We test this idea on a model that generates {\it scripts} (event sequences), to see if an error corrector model can learn
% to repair script errors (e.g., wrong event ordering) from a user's NL feedback. Our results show that the trained model can then interpret user feedback about new scripts, resulting in scripts.
% we also describe ongoing work on adding a memory of users' feedback, so that the model can recall old problems (corrections) that occur in new examples, and correct those also, paving a path towards continuous improvement with progressively less feedback.
% % The system is trained over a new crowdsourced dataset with 1000 training examples that include natural feedback. This system paves the path towards continuous improvement with progressively less feedback, without retraining.
% \end{abstract}



% missing_step	['1. get out of car', '2. stop in front of car', '3. turn body towards back of car', '4. walk to back of car', '5. take blanket out of car', '6. walk to desired location', '7. throw blanket down']	a person needs to open the door before they take an object out'	insert node 'open the back door of the car' before 'take blanket out of car'	insert node 'open car door' before 'take blanket out of car'
% missing_step	['1. buy a video game', '2. talk to the cashier', '3. make the transaction', '4. get the receipt', '5. load the video game into the car', '6. get into the car', '7. take xbox home']	after a person makes a transaction, they then head to their car'	insert node 'walk to the car' after 'get the receipt'	insert node 'get into the car' after 'make the transaction'
% wrong_step	['1. warm up in locker', '2. adjust gym gear', '3. shake body out', '4. face the locker room', '5. walk towards the locker room', '6. open the locker room door', '7. change into a fresh outfit', '8. walk to the locker room', '9. walk to locker room']	can't go where you already are"	remove node 'walk to the locker room'	reorder edge between '$\langle$ walk towards the locker room , walk to the locker room $\rangle$'
% wrong_step	['1. make a bunch of cards', '-- 2. grab a pen', '-- 3. grab some paper', '4. pick up a pen', '5. place the paper on the table', '6. pick up the pen', '7. write names on the cards']	good plans shouldn't include redundant steps"	remove node 'pick up the pen'	remove node 'pick up a pen'
% wrong_ordering	['1. grab the blind cords', '2. walk to the window', '3. place hands on blinds', '4. hold the blind cords', '5. push blinds up', '6. pull blinds up', '7. lift the blinds up']	you have to be near something to grab it'	reorder edge between '$\langle$ grab the blind cords , walk to the window $\rangle$'	reorder edge between '$\langle$ walk to the window , grab the blind cords $\rangle$'
% wrong_ordering	['1. leave home and get in car', '2. remember the address of the destination', '3. look around for the car', '4. walk towards the car', '5. open the car door', '6. sit down in the car', '7. put on the seatbelt', '8. enter car and fasten seat belt']	you wouldn't look for something you're already with"	reorder edge between '$\langle$ leave home and get in car , look around for the car $\rangle$'	remove node 'look around for the car'Z



\begin{tikzpicture}
\begin{axis}[
	xlabel=put ur xlabel,
	ylabel=put ur ylabel,
	width=10cm,height=7cm,
    legend style={at={(0.0,.91)},anchor=west}]
\addplot[color=red,mark=x] coordinates {
	(1, 7)
	(2, 8)
	(3, 9)
	(4, 10)
	(5, 11)
	(6, 12)
};

\addplot[color=blue,mark=*] coordinates {
	(1, 9)
	(2, 10)
	(3, 11)
	(4, 12)
	(5, 13)
	(6, 14)
};

\legend{Case 1,Case 2}
\end{axis}
\end{tikzpicture}





==> sections/interscript_data_collection.tex <==
\section{\ours collection}


We believe that an average user could point out mistakes in the generated scripts, as a majority of the errors in generated scripts are caused by a lack of basic commonsense~(\S{\ref{sec:subsec:study}}).
Consequently, we designed a Mechanical Turk task to provide feedback on mistakes.  A broad overview of the annotation process is shown in Figure \ref{fig:mturk-idea}. \am{This paragraph can be at the end of revised Section 3 (we discuss the design of our annotation process next...)}

\begin{figure}[!ht]
\centering
{\includegraphics[width=0.9\columnwidth]{imgs_v2/data-collection-overview.pdf}}
\caption{A broad overview of the annotation process. For actual annotation task (including the M-turk task template), see our code repository.
%Specific Mechanical Turk instructions and sample annotation pages are provided in the anonymously released code repository.
}
\label{fig:mturk-idea}
\end{figure}

\paragraph{Annotation}
Now we discuss our crowdsourcing setup to collect \ours. To maximize the opportunity to get more feedbacks for a predicted script, we filtered a subset of the test set in ProScript where the human evaluated graph edit distance was likely to be high (i.e., there were likely to be more errors). The ProScript authors released the graph edit value for the set of test set samples they evaluated. We performed inference using their released \proscriptgen model on those data points with high graph edit distance value ($\ge 8$). With this we collected about 400 (predicted graph, expected gold graph) tuples. The ProScript paper describes that their expected gold graph is also imperfect and might contain about 20\% noise. 
Nevertheless, having the gold reference graph guides and constrains an annotator about the common script for a scenario rather than the wide open space of solving the task using multiple potentially correct scripts. (e.g., one could go to a zoo without driving the car by hiring a taxi and then they won't need to drive or park the car). 
As mentioned in \S{\ref{sec:subsec:study}} our annotation process must focus on scripts that are widely applicable and grounded in commonsense.

The annotators are shown the model-generated and expected gold (reference) scripts, and are required to answer which script is worse and why.
It is possible that the gold script is marked as worse.
However, we later post-process and remove such cases, as our focus is to get errors on the generated scripts and not the manually created scripts.
The annotators must point out an egregious \corr{egregious}{obvious} mistake (\eg an event or an edge that does not follow commonsense).
%, and trivial errors like minor grammatical mistakes)
They were asked to ignore grammatical and fluency errors, and focus on critical errors of four types:
\squishlist
\item \textbf{Wrong ordering:} the order in the sequence of steps is not correct (\eg wearing shoes is described before wearing socks).
\item \textbf{Flexible ordering:} some steps can be done in a flexible order (\eg you can wear left sock or right sock first). A good script captures such flexibility.
\item \textbf{Missing critical steps:} a bad script might have missed critical steps (\eg the script can say: ``wait for a plane'' followed by ``get off the plane'' -- here an obvious step ``get on the plane" is missing) . There is no strict definition for a critical step, so the annotators were instructed to use their commonsense judgment.
\item \textbf{Wrong step:} a bad script might have irrelevant and wrong steps (\eg the script describing ``go to a party" might describe an irrelevant step such as read a book, open a book, etc.).
\squishend


For every data point, the annotators were asked to answer the following: 
\squishlist
    \item Explicit feedback type-1: the error type (missing step, wrong step, wrong order, wrong partial order)
    \item Explicit feedback type-2: localize the error by providing the erroneous node or edge id
    \item Implicit feedback type-1: give feedback in a few words, explaining the error
    \item Implicit feedback type-2: An explanation of the error that would potentially make sense to a five-year-old. This was aimed to explain the feedback to gather the general principle behind the feedback.
\squishend
\am{Are these labels (Explicit feedback type-1/2) wrong? Can we just call them \textit{error type, location, feedback, and explanation}?}
Fig. \ref{fig:mturk-page} shows a sample of our Mechanical Turk task.


Annotators were required to list only one critical error that they believe was most important.
Each data point is annotated by three annotators, adding some diversity in the errors. 
The annotators were paid \$15 an hour.
\corr{Estimated}{The average} time for completion of one script was 2 minutes. 
\corr{We monitored all the jobs via comments, and the annotators did not raise any concerns about the pay or the nature of the task or its difficulty.}{}

We measured the agreement on labels (which graph is worse), and on explicit feedback type-1 and type-2. It was difficult to measure agreement on implicit feedback because it is not easy to perform binary comparison on the generated text without accounting for linguistic variations. On the labels, the Fleiss Kappa agreement was 0.90 (almost perfect agreement) and on explicit feedback the agreement was 0.75 Fleiss Kappa (substantial agreement). This also shows that there is some diversity in what the users perceive as a serious mistake in \badgm. 

Eventually, we compiled these annotations into a dataset of 1,553  4-tuples where each entry consists of (explicit feedback type-1, explicit feedback type-2, implicit feedback type-1, implicit feedback type-2). 




\paragraph{Distractor feedback}
We also add distractor feedbacks, these are cases when the feedback does not apply to the graph. This covers the real-world scenario when a user gives an irrelevant feedback, then an interactive model must be convinced that the feedback is not applicable. To do this, we find the top-k neighbors of the input graph and rest of the graphs by encoding the graphs using Sentence transformers~\citep{reimers-2019-sentence-bert}, and then compute cosine distance. To get irrelevant but lexically related feedback, we attached the feedback of the least similar example (at rank=k and k-1). By random sampling we manually found that k=4 gives reasonable lexical similarity but the feedback are not applicable across the scripts. This subset gives us another approximately 2,026 instances. % 791 top4, 1235 top3


% The following step is not right: put the shirt on
% Remove node 'put the shirt on'
% It tells you to iron your shirt while it's still on your body.
% If you hold a hot iron against the clothes you're currently wearing, you'll get terrible burns.
\paragraph{Shared feedback}
We often encounter recurring themes or nearly similar situations, and these pairs should share much of their feedback. For example, suppose the goal is to buy grocery and the generated graph is missing an important step like pay for the item. In that case, we can synthesize new examples from it by replacing ``grocery'' with ``toilet paper'' or ``clothes'' in the tuple (\badgm, \fbm, \corrgm).
We manually label a subset of 50 examples by substituting a word in the goal and creating a new tuple. 

We compile these data points into 8,466 samples -- each sample is a tuple (\badgm, \fbm, \corrgm). Table \ref{tab:dataset_statistics_by_feedback_type} breaks down the total number of samples by feedback type. 

\am{The shared and distractor feedback might be better suited for the experiments, especially because they are not available for each sample. Also, why is the number of distractor fb 1553? My understanding is that we can generate a distractor feedback for every graph}

\begin{table}[!h]
   \small
    \centering
    \begin{tabular}{|p{0.2\columnwidth}|p{0.1\columnwidth}||p{0.58\columnwidth}|}
    \hline \fbm type &  count & example \\ \hline
explicit \fbm type-1 & 1,553 & Remove node `put the shirt on' \\ \hline
explicit \fbm type-2 & 1,553 & The following step is not right: put the shirt on \\ \hline
implicit \fbm type-1 & 1,553 & It tells you to iron your shirt while it's still on your body. \\ \hline
implicit \fbm type-2 & 1,553 & If you hold a hot iron against the clothes you're currently wearing, you'll get terrible burns. \\ \hline
distractor \fbm      & 2,026 & People do not use two scissors at a time, they simply use one\\  \hline
shared \fbm     & 228   & (illustrative) It tells you to iron your pant while it's still on your body\\ \hline  
total & 8,466 & \url{https://anonymous.4open.science/r/interscript/data.json} \\ \hline
    \end{tabular}
    \caption{\ours dataset statistics. \am{The examples are not very helpful without the accompanying script. Perhaps we can move the larger table to the appendix, and only retain a table of counts here.}}
    \label{tab:dataset_statistics_by_feedback_type}
\end{table}


%We next describe two scenarios where it can potentially advance the field.






% done
% \am{We should add a paragraph somewhere in the paper to address arguments of the nature: \textit{but what if someone drives to the zoo to get in another car?} The argument is simple; our goal is not to generate scripts that contain every possible outcome or outlying event. Rather, we aim to generate widely applicable scripts and grounded in commonsense.}



% Less Non-critical errors: These characteristics do not define a worse plan::
% Grammatical and fluency errors: a bad script usually has less fluent steps or contains many grammatical mistakes.
% Redundant steps: some steps in the script might have redundant steps, e.g., step 3 and step 4 might repeat.
% Granularity: note that a more fine-grained script is not a worse script (e.g., go the bed, get up, brush vs. get up, get ready)





% You have to justify why that script is worse.
% Type of error: One of
% wrong ordering
% incorrect flexible ordering
% wrong step
% missing step
% step number: i.e., which step or edge is wrong, (e.g., 4-5 indicates edge from step 4 to step 5 is wrong). When referring to a pair of steps (e.g., one should happen after the other) then please write them separated by comma e.g., 4-5, 6-7
% reason: why is that edge or step wrong? (describe in some detail, very short answers are not accepted.)
% principle: what is the general principle/ rule of thumb behind your reason? If you were to explain your reason to a five-year-old, how would you do that with general principles/ commonsense facts? (describe in some detail, very short answers are not accepted.)







==> sections/interscript_data_task_overview.tex <==
% script generation task.
% model, we made inference on.
% what authors claim and also what we found is that errors exist but are not all over the place.
% but while the evaluators/ turkers could tell the error, the model doesn't react.
% This is the motivation for our dataset for interactive learning with proscript_gen output as the starting point.

\section{Script generation}
Complex everyday events, such as visiting a restaurant, can typically be described as a sequence of distinct sub-events and actions.
Scripts~\citep{Schank1975ScriptsPA} are an efficient way of capturing information about the sub-events and sequences that form a complex event.
A prominent example of scripts in a modern context is their use in digital assistants like Siri, which organize common tasks such as setting up a reminder in script-like workflows~\citep{learning-decompose-tasks-2021}, \corr{The eventual goal of this work is...}{or for an agent in an environment  \cite{Shridhar2020ALFRED}, to execute a task by following a script or even generating a script itself.}


% \corr{People use task management applications with digital assistants such as Siri to organize, track, and complete tasks at work and outside of work.}{}
% \citep{learning-decompose-tasks-2021}

% agreed: dropping this and adding a line in the previous.
% The eventual goal of this line of work is, given a goal plan, to execute in a real-world or virtual environment such as ALFRED \cite{Shridhar2020ALFRED}. An intermediate step to reach there is to generate the script given a task such as ``bake a cake'', ``fix a bike tire'' or ``fuel a car''.\am{Can drop this paragraph} 

\subsection{Script generation}
Formally, the script generation task \cite{proscript} takes as input a scenario and generates a script $G(V, E)$, where $V$ is a set of essential events $\{v_1, ... v_i, ... v_{|V|}\}$ and $E$ is a set of temporal ordering constraints between events $\{e_{ij}\}$ which means that the events $v_i$ must precede the event $v_j$ ($v_i \prec v_j$). Partial ordering of events is possible, e.g., you can wear a left sock and a right sock in any temporal order. To solve this task, script generation models are required to \textit{generate} events ($V$) and predict the edges ($E$) jointly. See Figure \ref{fig:proscript_orig_example} for an example.

\begin{figure}[!ht]
\centering
{\includegraphics[width=0.8\columnwidth]{imgs/proscript.pdf}}
\caption{An example of a \textit{script} in \citet{proscript}. In a script generation task, models take the goal as the input and generate a (possibly) partial-order graph, which consists of essential steps and their ordering.}
\label{fig:proscript_orig_example}
\end{figure}

\proscriptgen  \cite{proscript} is a recently released model that, given a goal, generates $V$ and predicts the edge structure $E$ jointly. It is based on the T5-XXL model (11B parameters) and generates the script as a graph in DOT format. The authors report that the DOT format is always valid at inference time and that $V$ and the graph structure are generally of high quality. They characterize the graph edits required to correct a generated script (such as removing a node, adding a node, changing edge order, etc.). Mechanical Turk workers were able to correct most of the generated scripts within a few edits (typically an edit distance of 5). This makes for an attractive use-case for interactive learning because the generated content from the model (i) is not completely off and (ii) naturally exposes its belief/understanding of the goal through the edge structure, and a user can critique or provide feedback on this belief. 
\am{I think the rest of the section can be deleted/shortened to a paragraph. Essentially, all we need to say is: i) There is a script generation model, ii) it makes mistakes on which it is possible to provide feedback. Then, we can directly start from section 4 on collecting this feedback.}


\subsection{Initial study}
\label{sec:subsec:study}
How do the corrective edits typically look like? On ProScript's test set, we performed inference using the released checkpoint (both GPT-2 and T5-XXL based model). We randomly sampled 30 generated graphs and manually wrote feedback for them (see Table \ref{tab:study-sample-feedback}). 
On average, there were about two mistakes present in the graphs. Often, the error was that the script was using an entity before having it (e.g., write on the paper comes before the node find the paper or reach for the paper). 
Thus, there seems to be a possibility of applying similar feedback to more than one example.
%something more systematic, but we did not do more model analysis; rather, we noted that having general level feedback is possible. 
We also found some cases where the script might have to be changed to adapt to special cases. 
For example, for a script \textit{visit Disneyland}, an event \textit{obtain a visa} might be required for some users.
%, e.g., visa requirements to travel somewhere. 
We believe the original ProScript dataset aims to generate widely applicable scripts and grounded in commonsense; rather than cover all possible outcomes. 

% \am{In the intro, we are saying that 20\% of the scripts had errors. I don't see that number here. Maybe there is a discrepancy?}
% answer: I meant 10% within the erroneous instances.

% Most frequent: ~10% instances had the following error. (using something before having it)
% You need to have an object before using it. (eg. write on the paper comes before to find the paper or reach for the paper)
% You must find something before accessing it.
% You need to perform an action only once. (e.g., sitting on a chair twice)
% etc. 

% 57 (edge issues)
% 16 (node issues missing step)
% 27 (wrong step)
\begin{table}[!h]
    \centering
    \begin{tabular}{|p{0.46\columnwidth}|p{0.46\columnwidth}|}
    \hline \textbf{What was the error} &  \textbf{General principle feedback} \\ \hline
    Script was missing the step of not turning off the alarm after waking up & People don't leave their alarms ringing all day.\\ \hline
    Script mentioned coming to the doorway and passing through it & One cannot walk through the doorway without opening the door first. \\ \hline
    \end{tabular}
    \caption{Sample feedback on the examples in the study.}
    \label{tab:study-sample-feedback}
\end{table}


\subsection{Conclusions from the initial study}

On the surface, the generated scripts were of good quality.
However, a closer look at the mistakes revealed that most of them could be attributed to the model lacking basic commonsense. 
For example, Figure \ref{fig:intro-example} shows a typical mistake the model makes. 
This underscores the gap between the syntax and semantic correctness of machine-generated output in the context of automatic script generation. 
This observation is in-line with other NLP tasks \citep{BenderKoller2020FormAndMeaning} that distinguish the success of recent models on the correctness of form rather than the far-from-over goal of understanding of meaning.

We had two questions: (i) Is there a set of general commonsense principles that the model fails to adhere to. (ii) How can the model incorporate simple feedback and improve? It is costly to retrain large LMs such as the T5-XXL model, and we hoped to make a new component that learns to take feedback from a user. However, we could not find any dataset to solve such an interactive learning problem. Despite recent progress in synthetic or constrained settings, a real-world dataset in a structured prediction setting does not exist. Like with this example, structured prediction models can generate inconsistent output, ignoring the structural complexity of human language. Their decoding is typically based on greedy or sample decoding, and structural incoherence is a possibility. If such a dataset exists with feedback on the generated structure, it would help improve structured outputs-- a widespread problem.
How can an end-user provide feedback if a deployed structured prediction model generates inconsistent output,  ignoring the structural complexity of human language? This is an emerging topic with recent progress in synthetic or constrained settings, and the next big leap would require testing and tuning models in real-world settings. We present a new dataset, \ours, containing user feedback on a deployed model that generates complex everyday tasks. \ours\footnote{Code \& data:  \url{https://anonymous.4open.science/r/interscript}} contains 8,466 data points-- the input is a possibly erroneous script and a user feedback and the output is a modified script. 
We posit two use-cases of \ours that might significantly advance the state-of-the-art in interactive learning.

==> sections/introduction-old-v1.tex <==

\section{Introduction}

While language models have achieved remarkable performance on several reasoning tasks \cite{Wang2018GLUE, talmor-etal-2019-commonsenseqa}, they are still prone to mistakes \citep{BenderKoller2020FormAndMeaning}. 
This is especially true in structured prediction settings because models can ignore the structural complexity of human language, and rely on simplistic and error-prone greedy search procedures \cite{martins2020deepspin}. 
As a result, these models typically produce syntactically correct output structures but have commonsense issues that degenerate the output \cite{proscript}. 
In deployed models, end-users can report such commonsense issues and inconsistency errors in the generated output structures, but retraining these models is prohibitively costly.

\begin{figure}[!t]
\centering
%    {\includegraphics[width=\columnwidth]{acl-ijcnlp2021-templates/imgs/example-graph.png}}
%    {\includegraphics[width=\columnwidth]{acl-ijcnlp2021-templates/imgs/stages2.png}}
 %   {\includegraphics[width=\columnwidth]{imgs_v2/running_example.pdf}}
      {\includegraphics[width=\columnwidth]{imgs_v2/revised-running-example.png}}
   \caption{
     Given a frozen model \basemodelm, we train a {\it corrector model} G to
     apply feedback from a user about errors made by the original model. In the example,
     \basemodelm has generated a script with an error in, stating that ``driving'' and
     ``getting in a car'' can occur in any order (red box). The user provides general feedback
     (``Get in a car before driving''), and G operationalizes this to
     generate a corrected graph (by predicting and applying a graph edit operation) in which ``get in car'' happens first (green box). The feedback is stored in memory M so it can also be retrieved to repair similar, future errors.}
\label{fig:intro-example}
\vspace{-3mm}
\end{figure}


Our goal is to allow users to correct such errors directly through interaction,  without retraining -- by giving feedback on the model's output or explanation.
We consider the class of problems where the model's structured output is a \textit{graph} of nodes and edges.
Graphs have a rich structure and capture complex interactions between nodes. 
Consequently, graphs generated by models often have issues that an end user can highlight.
Specifically, we find that current seq2seq models typically produce syntactically correct output structure but have commonsense issues that degenerate the output \cite{proscript}, and end-users can critique such commonsense issues via natural feedback \cite{Talmor2020TeachingPM}. 
Given a partially incorrect structure and end-user feedback, we aim to localize an erroneous node or edge in the graph and generate a repaired graph. 
Learning to repair structure poses two major challenges: First, the system needs to connect and jointly reason over the incorrect source structure and the user feedback. 
Second, existing works that do structured generation do not account for end-user feedback after deployment \cite{Yasunaga2020Bifi-v0-PercyLiang,yasunaga2021break}.
%\am{we can cite our graph generation works}
% \am{The next part breaks the flow. We need to transition or move this above}
Our key innovation is doing structured output repair using feedback by an end-user.
% \am{This sentence has a lot of words we have not defined yet}





% End users typically may not know the completely correct output structure but can critique any inconsistencies or commonsense issues in partially correct output structures (common in practice). 

Our approach loosely follows some early AI systems that maintained a memory of output problems and how to fix them~\citep{Sussman1973ACM, Hammond1986CHEFAM, Riesbeck1981FailureDrivenRF},
but here we use neural methods and interact with a user to provide corrective feedback.
% HACKER \cite{Sussman1973ACM}, Chef \cite{Hammond1986CHEFAM}, and the
% broader research area of failure-driven reminding \cite{Riesbeck1981FailureDrivenRF}.
% However, these did not involve user interaction and feedback.
More recently, it has been shown that neural methods can use expert feedback that guides the model towards the gold output in specialized domains (e.g., SQL experts' feedback for natural language database query parsing \citep{elgohary2021nl}; and compiler feedback for code fixing in  \citet{Yasunaga2020Bifi-v0-PercyLiang}). 
% However, the assumption of having expert feedback in specialized domains limits the generality of these approaches. 
In contrast, in our work corrections by an end-user are expressed in a {\it general} way that also applies to new problems, as the model learns to operationalize those corrections.
% \am{I think we have two different advantages over these methods: i) The feedback is not example specific, ii) we don't need experts. I think the previous two paragraphs mix these points. At the same time, they are perhaps coupled (if example is specific to a sample, maybe the task is so challenging that we need experts).}


Our approach is to add a {\it corrector module}, operating on the original model's output. %\corr{}{Then, through a multi-tasking objective, the corrector module is trained to perform two different tasks: i) to generate the output structures, and ii) to interpret natural language feedback from the user and correct a noisy output using it.} %Then, through a multi-tasking objective, 
The corrector module is trained to interpret natural language feedback from the user and correct that output using it and do the original task of generating output structures (that can be noisy).
In particular, our goal is for user feedback to be general, applied to multiple samples, rather than specific edit operations on particular model output.
We address this by introducing a \textit{dynamic memory} of user interactions for an error scenario, so that feedback on one problem can also be used to correct future, similar problems.


To validate our approach, we use a recently published dataset, \iscript \citep{interscript}, containing tuples of an imperfect generated script, a piece of user feedback, and a revised script, where a script is a graph of events and their temporal ordering describing how to achieve a given goal.
On this challenging task, we show that \ours can revise the scripts using natural feedback, leading to 10x improvement over a baseline that does not uses feedback. 
We also show that our memory architecture is effective as it improves performance by 10\% on unseen instances by growing and using the memory after deployment.
The empirical evidence and ideas presented in this work are a first step towards strengthening deployed large-scale models, potentially broadening their utility. 



% \niket{if a graph had multiple errors, batch mode or one by one by breaking when there are multiple feedbacks. Discuss multitasking setup.}
% While language models have achieved remarkable performance, they still make mistakes. \niket{add some references}
% Given an erroneous output, our goals are two-fold: First, to enable the user to teach the
% machine what the problem is in a {\it natural, general} way. Second, for the machine to
% also apply that feedback to {\it new} problems, so its performance continuously improves
% with time. We describe experiments for first goal, and work in progress towards the
% second goal.

% Our approach is to add a {\it corrector module}, operating on the original model's
% output. The corrector module is trained to interpret natural language feedback from
% the user, and how to correct that output using it. In particular, our goal is for
% user feedback to be general, that can be applied to multiple problems, rather than
% specific edit operations on a particular model output. If this can be achieved, it
% paves the path towards continuous improvement over time, without retraining.

% We develop this approach for an existing model, called proScript \cite{proscript}, although
% our approach can be applied to any model producing structured output.
% proScript takes as input a goal to achieve (expressed in NL), and outputs a
% partially ordered sequence of steps - a {\it script} - required to achieve
% that goal. Our interest here is not in proScript itself, but what to do
% when proScript's output contains an error.

% Our general approach, and a specific example for proScript, is shown in
% Figure~\ref{fig:intro-example}. In this example, proScript's original
% output script contains an error: it states that the steps of ``driving''
% and ``get in car'' can be applied in any order. The user provides general
% feedback ``Get in a car before driving''. The corrector model $\mathcal{G}$ then
% takes that feedback and the original script, and applies it to generate
% a corrected script. We also explore drawing feedback from a {\it persistent memory}
% of prior feedback (rather than the user), using the new problem to find similar
% previous problems whose feedback may be applicable to the new problem also.

% % To train G, we use a dataset of examples of
% % bad scripts, feedback, and corrected scripts. Given this training,
% % G aims to interpret new feedback for new problems the user observes,
% % and correct them appropriately. We also speculate on storing user
% % feedback in a {\it memory}, so that appropriate feedback can be
% % automatically recalled and applied for new model outputs. For
% % example, if proScript makes a similar ordering mistake for a new
% % task, e.g., getting to work, the feedback ``Get in a car before driving''
% % would be recalled and applied to correct the error.

% Our approach loosely follows some early AI systems that maintained a memory of output problems
% and how to fix them, e.g., \cite{Sussman1973ACM,Hammond1986CHEFAM,Riesbeck1981FailureDrivenRF},
% but here we using neural methods, and interact with a user to provide corrective feedback.
% % HACKER \cite{Sussman1973ACM}, Chef \cite{Hammond1986CHEFAM}, and the
% % broader reseach area of failure-driven reminding \cite{Riesbeck1981FailureDrivenRF}.
% % However, these did not involve user interaction and feedback.
% More recently, NL-Edit loosely follows our architecture, allowing users to correct
% semantic parsing errors using natural language \cite{elgohary2021nl}. However,
% user corrections in NL-Edit are situation-specific, e.g., `''replace course id with program id.''
% In contract, our work here explores corrections expressed in a {\it general} way that can be applied
% to new problems also, with the model $\mathcal{G}$ learning to operationalize those corrections.

% \eat{
% Our goal is for a machine to learn from a user's feedback so that it continuously improves with time,
% without requiring expensive re-training at each step. In particular, we want the user's feedback to
% be {\it general}, so it can also be applied to new problems. Given a model $M$ that produces some
% (possibly erroneous) output, our approach is to add a {\it corrector model} that is 


% Teaching a machine via human instructions has long been a goal of AI, yet current neural methods typically require large numbers of examples to convey knowledge. Recently, LeapOfThought \cite{Talmor2020TeachingPM} instead taught pre-trained models on-the-fly using a few general statements without requiring re-training of the model. For the first time we \textit{attempt} to continuously teach a neural model through corrections on its output structure with a memory based architecture that avoids re-training. 
% }

% \eat{
% % Niket: An extended related work discussion here to dispense with the related work.
% A common theme in prior approaches to this task based on interactive semantic parsing (such as \cite{elgohary2021nl, percy-2016-learning-language-games-interaction-shouldrn}) is that user feedback is mapped into structure edit commands, which can then be executed on the incorrect structures to fix it. For example, \cite{elgohary2021nl} presented \nle to fix SQL queries using human feedback such as: 
% \texttt{replace course id with program id.}. 
% However:
% \squishlist
% \item the feedback are syntactic with a certain task-specific formal structure, e.g., \nle is known to struggle with natural feedback that does not describe an edit directly \cite{elgohary2021nl}.
% \item the feedback is expected to be actionable. Rather than highlighting a problem or error, it is expected to contain a solution to fix the error. This feedback is then parsed using semantic parsing techniques into a set of structure edit commands. 
% \item past feedback is discarded, and not used in future examples. In practice, a system often encounters recurring themes or situations, or nearly similar situations, e.g., \textit{people must get into a vehicle before driving to any place}. 
% \squishend

% Overcoming these problems, this paper does not make assumptions about the structure of the feedback and gives flexibility to a human to supply natural language instructions which could point out to some error and not necessarily edit specifications. This allows the editing operations to be inferred implicitly, triggered by the specification of the error. 

% We propose a pipeline system with two components, a previously trained neural model $\mathcal{M}$ and a graph corrector $\mathcal{G}$. The system takes as input any previously trained neural model $\mathcal{M}$ capable of generating a structured output. The second input is a natural language human feedback on the output structure (for an example, see Figure \ref{fig:intro-example}). As output, it produces a better structure, without retraining using a feedback table accessible through a memory layer.
% }


